Accelerating Recommendation System Training by Leveraging Popular Choices

Recommender models are commonly used to suggest relevant items to a user for e-commerce and online advertisement-based applications. These models use massive embedding tables to store numerical representation of items' and users' categorical variables (memory intensive) and employ neural networks (compute intensive) to generate final recommendations. Training these large-scale recommendation models is evolving to require increasing data and compute resources. The highly parallel neural networks portion of these models can benefit from GPU acceleration however, large embedding tables often cannot fit in the limited-capacity GPU device memory. Hence, this paper deep dives into the semantics of training data and obtains insights about the feature access, transfer, and usage patterns of these models. We observe that, due to the popularity of certain inputs, the accesses to the embeddings are highly skewed with a few embedding entries being accessed up to 10000x more. This paper leverages this asymmetrical access pattern to offer a framework, called FAE, and proposes a hot-embedding aware data layout for training recommender models. This layout utilizes the scarce GPU memory for storing the highly accessed embeddings, thus reduces the data transfers from CPU to GPU. At the same time, FAE engages the GPU to accelerate the executions of these hot embedding entries. Experiments on production-scale recommendation models with real datasets show that FAE reduces the overall training time by 2.3x and 1.52x in comparison to XDL CPU-only and XDL CPU-GPU execution while maintaining baseline accuracy

==> body/discussion.tex <==
\section{Discussion}
\todo{Prashant/Divya/Yassaman}{The goal here is to argue that we could have more datasets but they would have the same behavior and in production embedded tables are larger. Also, this should work with other models that use embedded tables as well}

==> body/tables/abs_training_time.tex <==
\begin{table}[h!]
\centering
\caption{Absolute Training Time}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
 \hline
 \textbf{Dataset} & \textbf{Baseline (min)} & \textbf{FAE (min)} & \textbf{Reduction in}  \\
 & & & \textbf{Training Time (min)}  \\
 \hline \hline
 Criteo Kaggle & 285.2 & 180.4 & 104.8 \\
 \hline
 Taobao Alibaba & 332.2 & 69.6 & 262.6 \\
 \hline
 Criteo Terabyte & 585.5 & 326.5 & 259.0 \\
 \hline
\end{tabular}}
\vspace{-0.2in}
\label{table:trainingtime}
\vspace{-0.2in}
\end{table}

==> body/tables/benchmarks.tex <==
\newcolumntype{?}{!{\vrule width 2pt}}
\setlength\extrarowheight{4pt}
\resizebox{1.9\columnwidth}{!}{
\begin{tabular}{|p{0.14\linewidth}|p{0.16\linewidth}||p{0.08\linewidth}|p{0.06\linewidth}||p{0.04\linewidth}|p{0.04\linewidth}||p{0.06\linewidth}|p{0.06\linewidth}|p{0.09\linewidth}||p{0.14\linewidth}|p{0.12\linewidth}|p{0.08\linewidth}|}
\hline
%
\multirow{2}{*}{\textbf{Workload}} & \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c||}{\textbf{Training Input}} & \multicolumn{2}{c||}{\textbf{Dataset Features}} & \multicolumn{3}{c||}{\textbf{Embedding Tables}} & \multicolumn{3}{c|}{\textbf{Neural Network Config}}
\\
\cline{3-12} & & \textbf{Number} & \textbf{Size} & \textbf{Dense} & \textbf{Sparse} & \textbf{Number} & \textbf{Size} & \textbf{Dimension} & \textbf{Bottom MLP} & \textbf{Top MLP} & \textbf{DNN}
\\
\hline
RMC1 (TBSM~\cite{tbsm}) & Taobao (Alibaba)~\cite{alibaba} & 10 M & 1 GB & 3 & 16 & 3 & 0.3 GB & 4.1M$\times$16 & 1-16 \& 22-15-15 & 30-60-1 & Attn. Layer \\
 \hline
RMC2 (DLRM~\cite{dlrm}) & Criteo Kaggle~\cite{criteokaggle} & 45 M & 2.5 GB & 13 & 16 & 26 & 2 GB & 10.1M$\times$16 & 13-512-256-64-16 & 512-256-1 & - \\
 \hline
RMC3 (DLRM~\cite{dlrm}) & Criteo Terabyte~\cite{criteoterabyte} & 80 M  & 45 GB  & 13 & 64  & 26  & 61 GB & 73.1M$\times$64 & 13-512-256-64 & 512-512-256-1 & - \\
 \hline
\end{tabular}}

==> body/tables/dataset_table.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|p{2cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
 \hline
 \multicolumn{4}{|c|}{Dataset Specification} \\
 \hline
 Dataset & Dense Features & Sparse Features & Sparse Feature Size \\
 \hline
 Criteo Kaggle & 13 & 26 & 16 \\
 \hline
 Criteo Terabyte & 13 & 26 & 64 \\
 \hline
 Alibaba & 1 & 3 & 16 \\
 \hline
\end{tabular}
\caption{}
\label{table:2}
\end{table}

==> body/tables/gpu_config.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|p{0.8cm}|p{1.8cm}|p{2cm}|p{1.8cm}|}
 \hline
 \multicolumn{4}{|c|}{Device Specification} \\
 \hline
 Device & Architecture & Local Storage & Communication Link \\
 \hline
 GPU & NVIDIA Tesla V100 & 16GB & NVLink\\
 \hline
\end{tabular}
\caption{}
\label{table:1}
\end{table}

==> body/tables/hardware_specs_table.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|p{3.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
 \hline
 \multicolumn{4}{|c|}{Hardware Specification} \\
 \hline
 Dataset & Dense Features & Sparse Features & Sparse Feature Size \\
 \hline
 Criteo Kaggle & 13 & 26 & 16 \\
 \hline
 Criteo Terabyte & 13 & 26 & 64 \\
 \hline
 Alibaba & 1 & 3 & 16 \\
 \hline
\end{tabular}
\caption{}
\label{table:3}
\end{table}

==> body/tables/model_specs_table.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|p{1.2cm}|p{1.5cm}|p{2.5cm}|p{2cm}|}
 \hline
 \multicolumn{4}{|c|}{Model Specification} \\
 \hline
 Model & No of Tables & Bot MLP & Top MLP \\
 \hline
 RM1 & 3 & 1-6 & 15-15 \\
 \hline
 RM2 & 26 & 13-512-256-64-16 & 512-256-1 \\
 \hline
 RM3 & 26 & 13-512-256-64 & 512-512-256-1 \\
 \hline
\end{tabular}
\caption{}
\label{table:1}
\end{table}
